Enhancing Mutual Trustworthiness in Federated Learning for Data-Rich Smart Cities

Federated learning is a promising collaborative and privacy-preserving machine learning approach in data-rich smart cities. Nevertheless, the inherent heterogeneity of these urban environments presents a significant challenge in selecting trustworthy clients for collaborative model training. The usage of traditional approaches, such as the random client selection technique, poses several threats to the system's integrity due to the possibility of malicious client selection. Primarily, the existing literature focuses on assessing the trustworthiness of clients, neglecting the crucial aspect of trust in federated servers. To bridge this gap, in this work, we propose a novel framework that addresses the mutual trustworthiness in federated learning by considering the trust needs of both the client and the server. Our approach entails: (1) Creating preference functions for servers and clients, allowing them to rank each other based on trust scores, (2) Establishing a reputation-based recommendation system leveraging multiple clients to assess newly connected servers, (3) Assigning credibility scores to recommending devices for better server trustworthiness measurement, (4) Developing a trust assessment mechanism for smart devices using a statistical Interquartile Range (IQR) method, (5) Designing intelligent matching algorithms considering the preferences of both parties. Based on simulation and experimental results, our approach outperforms baseline methods by increasing trust levels, global model accuracy, and reducing non-trustworthy clients in the system.

==> references.tex <==
@article{i1,
  title={A survey on federated learning: The journey from centralized to distributed on-site learning and beyond},
  author={AbdulRahman, Sawsan and Tout, Hanine and Ould-Slimane, Hakima and Mourad, Azzam and Talhi, Chamseddine and Guizani, Mohsen},
  journal={IEEE Internet of Things Journal},
  volume={8},
  number={7},
  pages={5476--5497},
  year={2020},
  publisher={IEEE}
}

@article{i2,
  title={Federated learning: Strategies for improving communication efficiency},
  author={Kone{\v{c}}n{\`y}, Jakub and McMahan, H Brendan and Yu, Felix X and Richt{\'a}rik, Peter and Suresh, Ananda Theertha and Bacon, Dave},
  journal={arXiv preprint arXiv:1610.05492},
  year={2016}
}

@article{i3,
  title={Advances and open problems in federated learning},
  author={Kairouz, Peter and McMahan, H Brendan and Avent, Brendan and Bellet, Aur{\'e}lien and Bennis, Mehdi and Bhagoji, Arjun Nitin and Bonawitz, Kallista and Charles, Zachary and Cormode, Graham and Cummings, Rachel and others},
  journal={Foundations and Trends{\textregistered} in Machine Learning},
  volume={14},
  number={1--2},
  pages={1--210},
  year={2021},
  publisher={Now Publishers, Inc.}
}

@inproceedings{p1,
  title={Communication-efficient learning of deep networks from decentralized data},
  author={McMahan, Brendan and Moore, Eider and Ramage, Daniel and Hampson, Seth and y Arcas, Blaise Aguera},
  booktitle={Artificial intelligence and statistics},
  pages={1273--1282},
  year={2017},
  organization={PMLR}
}


@inproceedings{r1,
  title={A trust and energy-aware double deep reinforcement learning scheduling strategy for federated learning on IoT devices},
  author={Rjoub, Gaith and Abdel Wahab, Omar and Bentahar, Jamal and Bataineh, Ahmed},
  booktitle={Service-Oriented Computing: 18th International Conference, ICSOC 2020, Dubai, United Arab Emirates, December 14--17, 2020, Proceedings 18},
  pages={319--333},
  year={2020},
  organization={Springer}
}

@article{r2,
  title={A mutual information based federated learning framework for edge computing networks},
  author={Chen, Naiyue and Li, Yinglong and Liu, Xuejun and Zhang, Zhenjiang},
  journal={Computer Communications},
  volume={176},
  pages={23--30},
  year={2021},
  publisher={Elsevier}
}

@article{r3,
  title={Fltrust: Byzantine-robust federated learning via trust bootstrapping},
  author={Cao, Xiaoyu and Fang, Minghong and Liu, Jia and Gong, Neil Zhenqiang},
  journal={arXiv preprint arXiv:2012.13995},
  year={2020}
}

@article{r4,
  title={Federated against the cold: A trust-based federated learning approach to counter the cold start problem in recommendation systems},
  author={Wahab, Omar Abdel and Rjoub, Gaith and Bentahar, Jamal and Cohen, Robin},
  journal={Information Sciences},
  volume={601},
  pages={189--206},
  year={2022},
  publisher={Elsevier}
}

@inproceedings{r5,
  title={Flchain: A blockchain for auditable federated learning with trust and incentive},
  author={Bao, Xianglin and Su, Cheng and Xiong, Yan and Huang, Wenchao and Hu, Yifei},
  booktitle={2019 5th International Conference on Big Data Computing and Communications (BIGCOM)},
  pages={151--159},
  year={2019},
  organization={IEEE}
}

@article{r6,
  title={FedMint: Intelligent Bilateral Client Selection in Federated Learning with Newcomer IoT Devices},
  author={Wehbi, Osama and Arisdakessian, Sarhad and Wahab, Omar Abdel and Otrok, Hadi and Otoum, Safa and Mourad, Azzam and Guizani, Mohsen},
  journal={arXiv preprint arXiv:2211.01805},
  year={2022}
}

@inproceedings{r7,
  title={Towards Bilateral Client Selection in Federated Learning Using Matching Game Theory},
  author={Wehbi, Osama and Arisdakessian, Sarhad and Wahab, Omar Abdel and Otrok, Hadi and Otoum, Safa and Mourad, Azzam},
  booktitle={GLOBECOM 2022-2022 IEEE Global Communications Conference},
  pages={01--06},
  year={2022},
  organization={IEEE}
}
% boot section related work
@article{r8,
  title={Fltrust: Byzantine-robust federated learning via trust bootstrapping},
  author={Cao, Xiaoyu and Fang, Minghong and Liu, Jia and Gong, Neil Zhenqiang},
  journal={arXiv preprint arXiv:2012.13995},
  year={2020}
}

@inproceedings{r9,
  title={FLOD: Oblivious Defender for Private Byzantine-Robust Federated Learning with Dishonest-Majority},
  author={Dong, Ye and Chen, Xiaojun and Li, Kaiyun and Wang, Dakui and Zeng, Shuai},
  booktitle={Computer Security--ESORICS 2021: 26th European Symposium on Research in Computer Security, Darmstadt, Germany, October 4--8, 2021, Proceedings, Part I},
  pages={497--518},
  year={2021}
}

@article{r10,
  title={Federated against the cold: A trust-based federated learning approach to counter the cold start problem in recommendation systems},
  author={Wahab, Omar Abdel and Rjoub, Gaith and Bentahar, Jamal and Cohen, Robin},
  journal={Information Sciences},
  volume={601},
  pages={189--206},
  year={2022},
  publisher={Elsevier}
}

% game theory related 
@article{r11,
  title={A robust game-theoretical federated learning framework with joint differential privacy},
  author={Zhang, Lefeng and Zhu, Tianqing and Xiong, Ping and Zhou, Wanlei and Philip, S Yu},
  journal={IEEE Transactions on Knowledge and Data Engineering},
  volume={35},
  number={4},
  pages={3333--3346},
  year={2022},
  publisher={IEEE}
}

@article{r12,
  title={Matching-theory-based low-latency scheme for multitask federated learning in MEC networks},
  author={Chen, Dawei and Hong, Choong Seon and Wang, Li and Zha, Yiyong and Zhang, Yunfei and Liu, Xin and Han, Zhu},
  journal={IEEE Internet of Things Journal},
  volume={8},
  number={14},
  pages={11415--11426},
  year={2021},
  publisher={IEEE}
}

@inproceedings{r13,
  title={Training task allocation in federated edge learning: A matching-theoretic approach},
  author={Kang, Jiawen and Xiong, Zehui and Niyato, Dusit and Cao, Zhiguang and Leshem, Amir},
  booktitle={2020 IEEE 17th Annual Consumer Communications \& Networking Conference (CCNC)},
  pages={1--6},
  year={2020},
  organization={IEEE}
}






@article{pf1,
  title={An endorsement-based trust bootstrapping approach for newcomer cloud services},
  author={Wahab, Omar Abdel and Cohen, Robin and Bentahar, Jamal and Otrok, Hadi and Mourad, Azzam and Rjoub, Gaith},
  journal={Information Sciences},
  volume={527},
  pages={159--175},
  year={2020},
  publisher={Elsevier}
}


@article{fashion,
  title={Fashion-mnist: a novel image dataset for benchmarking machine learning algorithms},
  author={Xiao, Han and Rasul, Kashif and Vollgraf, Roland},
  journal={arXiv preprint arXiv:1708.07747},
  year={2017}
}

% recently added
@inproceedings{ahmad,
  title={Data-driven federated autonomous driving},
  author={Hammoud, Ahmad and Mourad, Azzam and Otrok, Hadi and Dziong, Zbigniew},
  booktitle={Mobile Web and Intelligent Information Systems: 18th International Conference, MobiWIS 2022, Rome, Italy, August 22--24, 2022, Proceedings},
  pages={79--90},
  year={2022},
  organization={Springer}
}

@article{arafeh,
  title={ModularFed: Leveraging modularity in federated learning frameworks},
  author={Arafeh, Mohamad and Otrok, Hadi and Ould-Slimane, Hakima and Mourad, Azzam and Talhi, Chamseddine and Damiani, Ernesto},
  journal={Internet of Things},
  pages={100694},
  year={2023},
  publisher={Elsevier}
}

@article{mario,
  title={On the feasibility of Federated Learning towards on-demand client deployment at the edge},
  author={Chahoud, Mario and Otoum, Safa and Mourad, Azzam},
  journal={Information Processing \& Management},
  volume={60},
  number={1},
  pages={103150},
  year={2023},
  publisher={Elsevier}
}

@article{sarhad,
  title={Coalitional Federated Learning: Improving Communication and Training on Non-IID Data with Selfish Clients},
  author={Arisdakessian, Sarhad and Wahab, Omar Abdel and Mourad, Azzam and Otrok, Hadi},
  journal={IEEE Transactions on Services Computing},
  year={2023},
  publisher={IEEE}
}

@article{omar,
  title={Intrusion detection in the iot under data and concept drifts: Online deep learning approach},
  author={Wahab, Omar Abdel},
  journal={IEEE Internet of Things Journal},
  volume={9},
  number={20},
  pages={19706--19716},
  year={2022},
  publisher={IEEE}
}

@article{waz,
  title={Warmup and Transfer Knowledge-Based Federated Learning Approach for IoT Continuous Authentication},
  author={Wazzeh, Mohamad and Ould-Slimane, Hakima and Talhi, Chamseddine and Mourad, Azzam and Guizani, Mohsen},
  journal={arXiv preprint arXiv:2211.05662},
  year={2022}
}

@article{mohsen,
  title={Fedgan-ids: Privacy-preserving ids using gan and federated learning},
  author={Tabassum, Aliya and Erbad, Aiman and Lebda, Wadha and Mohamed, Amr and Guizani, Mohsen},
  journal={Computer Communications},
  volume={192},
  pages={299--310},
  year={2022},
  publisher={Elsevier}
}

@article{hani,
  title={Opportunistic UAV Deployment for Intelligent On-Demand IoV Service Management},
  author={Sami, Hani and Saado, Reem and El Saoudi, Ahmad and Mourad, Azzam and Otrok, Hadi and Bentahar, Jamal},
  journal={IEEE Transactions on Network and Service Management},
  year={2023},
  publisher={IEEE}
}

@article{adoom1,
  title={TrustSys: Trusted Decision Making Scheme for Collaborative Artificial Intelligence of Things},
  author={Rathee, Geetanjali and Garg, Sahil and Kaddoum, Georges and Choi, Bong Jun and Hassan, Mohammad and Alqahtani, Salman A},
  journal={IEEE Transactions on Industrial Informatics},
  year={2022},
  publisher={IEEE}
}

@article{adoom2,
  title={Toward Accurate Anomaly Detection in Industrial Internet of Things Using Hierarchical Federated Learning},
  author={Wang, Xiaoding and Garg, Sahil and Lin, Hui and Hu, Jia and Kaddoum, Georges and Piran, Md Jalil and Hossain, M Shamim},
  journal={IEEE Internet of Things Journal},
  volume={9},
  number={10},
  pages={7110--7119},
  year={2021},
  publisher={IEEE}
}

@article{quinlan1986induction,
  title={Induction of decision trees},
  author={Quinlan, J. Ross},
  journal={Machine learning},
  volume={1},
  pages={81--106},
  year={1986},
  publisher={Springer}
}

@article{rabab1,
  title={A matching game-based crowdsourcing framework for last-mile delivery: Ground-vehicles and unmanned-aerial vehicles},
  author={Abualola, Huda and Mizouni, Rabeb and Otrok, Hadi and Singh, Shakti and Barada, Hassan},
  journal={Journal of Network and Computer Applications},
  pages={103601},
  year={2023},
  publisher={Elsevier}
}

@article{jamal,
  title={Target localization using multi-agent deep reinforcement learning with proximal policy optimization},
  author={Alagha, Ahmed and Singh, Shakti and Mizouni, Rabeb and Bentahar, Jamal and Otrok, Hadi},
  journal={Future Generation Computer Systems},
  volume={136},
  pages={342--357},
  year={2022},
  publisher={Elsevier}
}

% 

@article{wahab2016towards,
  title={Towards trustworthy multi-cloud services communities: A trust-based hedonic coalitional game},
  author={Wahab, Omar Abdel and Bentahar, Jamal and Otrok, Hadi and Mourad, Azzam},
  journal={IEEE Transactions on Services Computing},
  volume={11},
  number={1},
  pages={184--201},
  year={2016},
  publisher={IEEE}
}

@inproceedings{wehbi2023towards,
  title={Towards Mutual Trust-Based Matching For Federated Learning Client Selection},
  author={Wehbi, Osama and Wahab, Omar Abdel and Mourad, Azzam and Otrok, Hadi and Alkhzaimi, Hoda and Guizani, Mohsen},
  booktitle={2023 International Wireless Communications and Mobile Computing (IWCMC)},
  pages={1112--1117},
  year={2023},
  organization={IEEE}
}

@article{abdulrahman2020fedmccs,
  title={FedMCCS: Multicriteria client selection model for optimal IoT federated learning},
  author={AbdulRahman, Sawsan and Tout, Hanine and Mourad, Azzam and Talhi, Chamseddine},
  journal={IEEE Internet of Things Journal},
  volume={8},
  number={6},
  pages={4723--4735},
  year={2020},
  publisher={IEEE}
}

@inproceedings{nishio2019client,
  title={Client selection for federated learning with heterogeneous resources in mobile edge},
  author={Nishio, Takayuki and Yonetani, Ryo},
  booktitle={ICC 2019-2019 IEEE international conference on communications (ICC)},
  pages={1--7},
  year={2019},
  organization={IEEE}
}


@article{guesmi2023physical,
  title={Physical Adversarial Attacks For Camera-based Smart Systems: Current Trends, Categorization, Applications, Research Challenges, and Future Outlook},
  author={Guesmi, Amira and Hanif, Muhammad Abdullah and Ouni, Bassem and Shafique, Muhammad},
  journal={IEEE Access},
  year={2023},
  publisher={IEEE}
}
